Training-Free Hashing-Based Attention via Binary Principal Components

Long-context large language models (LLMs) are increasingly deployed in real-world applications, yet self-attention remains a major efficiency bottleneck -- especially during decoding -- due to the necessity of repeatedly processing ever-growing key-value (KV) caches. Existing sparse attention reduce computation by attending to fewer KV pairs, but often suffer from substantial accuracy degradation, require additional training, or rely on expensive hashing. In this work, we present BinaryPC, a training-free, data-aware hashing-based sparse attention for long-context LLMs. BinaryPC constructs compact binary hash codes and corresponding hash function by computing binary principal components of data. Unlike Locality-Sensitive Hashing (LSH) with data-independent random projections or learned non-linear hashing methods, BinaryPC constructs binary codes that explicitly preserve the structural information of data without requiring gradient-based training. Comprehensive experiments across multiple model families and long-context benchmarks show that BinaryPC preserves accuracy relative to full attention while achieving superior performance among sparse and hashing-based baselines. On modern GPUs, BinaryPC improves end-to-end decoding throughput by 3.56$\times$ over the FlashAttention kernel. Our code is available at https://github.com/yudaohai666/BPC.

==> figures/Longbench_llama38b_bar.tex <==
% Figure: Per-task breakdown on LongBench (Llama-3-8B)
\begin{figure}[htbp]
	\centering
    \includegraphics[width=\linewidth]{figures/LongBench_llama3-8b/longbench_bar.pdf}
	\caption{Per-task LongBench~\cite{bai2024longbench} breakdown on Llama-3-8B. BinVortex and Spotlight use a 2\% token budget and a minimum of 20 tokens; MagicPIG uses its default settings.}
	% 中文注释：Llama-3-8B 上 LongBench 分任务结果。BinVortex 和 Spotlight 使用 2\% 的 token 预算和最少保留 20 个 token；MagicPIG 使用其默认设置。
	\label{fig:longbench_llama38b_bar}
\end{figure}



==> figures/efficiency_ct.tex <==

\begin{figure}[t]
\centering
\begin{minipage}{0.48\linewidth}
    \centering 
    \includegraphics[width=\textwidth]{figures/efficiency/efficiency-batch-ct64K.pdf}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figures/efficiency/efficiency-batch-ct128K.pdf}
\end{minipage}
\caption{End-to-end throughput comparison across batch sizes (1--16) at fixed context lengths of 64K (left) and 128K (right) tokens.}
% 中文注释：在固定上下文长度（左：64K，右：128K）下，批量大小从 1 到 16 的端到端吞吐量比较。
\label{fig:efficiency_ct}
\end{figure}


==> figures/main_figure.tex <==
\begin{figure*}[!tb]
\centering
% \vspace{-0.05in}
\includegraphics[width=0.99\textwidth]{files/main-figure.pdf}
\vspace{-0.1in}
\caption{Overview of the BinVortex framework. (Left) During prefilling, BinVortex learns a data-aware binary projection matrix $\mP$ that maps key vectors to compact 64-bit hash codes $\mH$, explicitly minimizing the reconstruction error $\|\mK - \mH\mP\|_F$. (Middle) An error-aware safeguard identifies hard-to-quantize tokens with large residual norms and preserves them for reliable recall. (Right) During decoding, queries are projected via $\mP$ and binarized; top-$k$ keys are retrieved in Hamming space using GPU-friendly bitwise operations, enabling efficient sparse attention with approximately 2\% of full-attention cost.}
% 中文注释：BinVortex 框架概览。（左）在预填充阶段，BinVortex 学习一个数据感知的二值投影矩阵 $\mP$，将键向量映射为紧凑的 64 位哈希码 $\mH$，显式最小化重构误差 $\|\mK - \mH\mP\|_F$。（中）误差感知保障机制识别具有较大残差范数的难量化 token 并保留它们以确保可靠召回。（右）在解码阶段，查询通过 $\mP$ 投影并二值化；使用 GPU 友好的位运算在汉明空间中检索 top-$k$ 个键，从而以约 2\% 的全注意力开销实现高效稀疏注意力。
\label{fig:main_figure}
\vspace{-0.1in}
\end{figure*}


==> figures/verify.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/motivation/verify_motivation.pdf}
\caption{RULER~\cite{hsieh2024ruler} benchmark results from 8K to 128K context lengths. Both the TOPK and BinVortex adopt a 2\% token budget, while MagicPIG uses its default configuration.}
% 中文注释：RULER 基准在 8K 到 128K 的上下文范围内的结果。oracle TOP-$k$ 与 BinVortex 均使用 2\% 的 token 预算，而 MagicPIG 使用默认配置。
\label{fig:ruler_verify}
\end{figure}


==> tables/ablation__domain.tex <==
\begin{table}[!hptb]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \caption{Ablation study on OPC robustness under calibration-domain shift using LongBench~\cite{bai2024longbench}.}
  \label{tab:ablation_domain}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l|cccccc|c}
    \toprule
    Methods                 & S-Doc & M-Doc & Sum.  & F-shot & Syn.  & Code  & Avg. \\
    \midrule
    Full Attention          & 17.97 & 9.57  & 17.97 & 69.15  & 4.78  & 67.77 & 30.57 \\
    BinaryPC w/ OPC (mix)   & 17.78 & 9.66  & 17.50 & 69.10  & 5.44  & 66.66 & \underline{30.39} \\
    BinaryPC w/ OPC (PG19 only) & 18.26 & 9.47  & 17.78 & 68.92  & 4.71  & 67.06 & \textbf{30.43} \\
    \bottomrule
  \end{tabular}
  }
% \vspace{-0.1in}
\end{table}


==> tables/ablation_infinite.tex <==
\begin{table}[!hptb]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \caption{Ablation study on InfiniteBench with Llama-3.1-8B. We evaluate the effect of EAS.}
  \label{tab:ablation_infinite}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{l|c|ccccccc|c}
    \toprule
    Methods                  & EAS    & En.Sum& En.QA & En.MC  & En.Dia& Zh.QA  & Math.F& R.PK  & Avg. \\
    \midrule
    \textbf{Llama-3.1-8B}    & --   &32.13  &25.78  &69.00   &19.50  &31.90   &25.43  &99.32  &43.30 \\
    \midrule
    BinaryPC                 & yes   &33.06  &24.82  &69.00   &19.00  &31.87   &25.43  &99.32  &\textbf{43.21}  \\   
    BinaryPC w/ OPC          & yes   &32.61  &25.44  &69.00   &17.50  &32.35   &25.43  &99.32  &43.09 \\
    BinaryPC                 & no      & 31.89 & 25.75 & 69.00  & 17.00 & 30.71  & 24.29 & 55.76 & 36.34 \\
    BinaryPC w/ OPC          & no      & 32.46 & 26.30 & 69.00  & 17.50 & 31.81  & 25.43 & 99.32 & \underline{43.11} \\
    \bottomrule
  \end{tabular}
  }
\end{table}


==> tables/test.tex <==
\begin{table}[t]
  \caption{Classification accuracies for naive Bayes and flexible
    Bayes on various data sets.}
  \label{sample-table}
  \begin{center}
    \begin{small}
      \begin{sc}
        \begin{tabular}{lcccr}
          \toprule
          Data set  & Naive         & Flexible      & Better?  \\
          \midrule
          Breast    & 95.9$\pm$ 0.2 & 96.7$\pm$ 0.2 & $\surd$  \\
          Cleveland & 83.3$\pm$ 0.6 & 80.0$\pm$ 0.6 & $\times$ \\
          Glass2    & 61.9$\pm$ 1.4 & 83.8$\pm$ 0.7 & $\surd$  \\
          Credit    & 74.8$\pm$ 0.5 & 78.3$\pm$ 0.6 &          \\
          Horse     & 73.3$\pm$ 0.9 & 69.7$\pm$ 1.0 & $\times$ \\
          Meta      & 67.1$\pm$ 0.6 & 76.5$\pm$ 0.5 & $\surd$  \\
          Pima      & 75.1$\pm$ 0.6 & 73.9$\pm$ 0.5 &          \\
          Vehicle   & 44.9$\pm$ 0.6 & 61.5$\pm$ 0.4 & $\surd$  \\
          \bottomrule
        \end{tabular}
      \end{sc}
    \end{small}
  \end{center}
  \vskip -0.1in
\end{table}




